Gridless 2D Recovery of Lines using the Sliding Frank-Wolfe Algorithm

We present a new approach leveraging the Sliding Frank--Wolfe algorithm to address the challenge of line recovery in degraded images. Building upon advances in conditional gradient methods for sparse inverse problems with differentiable measurement models, we propose two distinct models tailored for line detection tasks within the realm of blurred line deconvolution and ridge detection of linear chirps in spectrogram images.

==> CommandesPerso.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%           Commandes perso            %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\matlab}{\textsc{Matlab}\texttrademark\xspace}

\newtheorem{remark}{Remark}

%% Figures centrées, et en position 'here, top, bottom or page'
\newenvironment{figureth}{%
		\begin{figure}[htbp]
			\centering
	}{
		\end{figure}
		}
		
		
%% Tableaux centrés, et en position 'here, top, bottom or page'
\newenvironment{tableth}{%
		\begin{table}[htbp]
			\centering
			%\rowcolors{1}{coleurtableau}{coleurtableau}
	}{
		\end{table}
		}

%% Sous-figures centrées, en position 'top'		
\newenvironment{subfigureth}[1]{%
	\begin{subfigure}[t]{#1}
	\centering
}{
	\end{subfigure}
}

\newcommand{\citationChap}[2]{%
	\epigraph{{\fontfamily{futs}\selectfont \og \textit{#1}\fg{}}}{#2}
}

%% On commence par une page impaire quand on change le style de numérotation de pages 
\let\oldpagenumbering\pagenumbering
\renewcommand{\pagenumbering}[1]{%
	\cleardoublepage
	\oldpagenumbering{#1}
}

\newcommand{\diff}{\mathop{}\mathopen{}\mathrm{d}}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\norme}[1]{\left\lVert#1\right\rVert}

\newcommand{\eu}{\ensuremath{\mathrm{e}}}
\newcommand{\jj}{\ensuremath{\mathrm{j}}}

\newcommand{\enquoted}[1]{\og #1\fg {}}


\newcommand{\expj}[1]{\ensuremath{\eu^{\, \jj #1}}}
\providecommand{\newoperator}[3]{%
	\newcommand*{#1}{\mathop{#2}#3}}
\providecommand{\renewoperator}[3]{%
	\renewcommand*{#1}{\mathop{#2}#3}}
\renewoperator{\Re}%
	{\mathrm{Re}}{\nolimits}
\renewoperator{\Im}%
	{\mathrm{Im}}{\nolimits}
	
\newcommand{\T}{\ensuremath{\mathsf{T}}}

\newcommand{\vect}[1]{\bm{#1}}
\newcommand{\mat}[1]{\mathbf{#1}}
\newcommand{\ten}[1]{\bm{\mathsf{#1}}}
\newcommand{\ope}[1]{\mathbf{#1}}
\newcommand{\ip}[2]{\left \langle #1\,,\, #2\right \rangle}
\newcommand{\RT}{\mathcal{R}}
\newcommand{\RTb}{\bm{\RT}}
\newcommand{\rtm}{\mathscr{R}}

% Full function
\providecommand{\fullfunction}[5]{\ensuremath{
   \begin {array}{ccccl}
       {#1}    & \colon  & {#2} & \longrightarrow & {#3} \\
       \mbox{} & \mbox{} & {#4} & \longmapsto     & {#5}
   \end{array}
}}
               
               
\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}







